Combined Task and Motion Planning Via Sketch Decompositions (Extended Version with Supplementary Material)

The challenge in combined task and motion planning (TAMP) is the effective integration of a search over a combinatorial space, usually carried out by a task planner, and a search over a continuous configuration space, carried out by a motion planner. Using motion planners for testing the feasibility of task plans and filling out the details is not effective because it makes the geometrical constraints play a passive role. This work introduces a new interleaved approach for integrating the two dimensions of TAMP that makes use of sketches, a recent simple but powerful language for expressing the decomposition of problems into subproblems. A sketch has width 1 if it decomposes the problem into subproblems that can be solved greedily in linear time. In the paper, a general sketch is introduced for several classes of TAMP problems which has width 1 under suitable assumptions. While sketch decompositions have been developed for classical planning, they offer two important benefits in the context of TAMP. First, when a task plan is found to be unfeasible due to the geometric constraints, the combinatorial search resumes in a specific sub-problem. Second, the sampling of object configurations is not done once, globally, at the start of the search, but locally, at the start of each subproblem. Optimizations of this basic setting are also considered and experimental results over existing and new pick-and-place benchmarks are reported.

==> sections/discussion.do.not.use.tex <==
%%% MOVED to experimental results
\Omit{

\begin{table*}[pt!]
    \newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
    \caption{Average results in the benchmarking problems.}\label{tab:solution}
    \centering
    \def\arraystretch{1.5}
    \setlength\tabcolsep{1mm}
    \begin{tabular}{|c|c|c|c|c||c|c|c|c|c|c|c|}
    \hline
    
    \makecell{Prob.} &
    \#Tables &
    \#Objects &
    \makecell{\#Goal\\objects} &
    \makecell{Clutter\\level} &
    Planner &
    \makecell{Success\\ratio} &
    \makecell{Planning\\time} &
    \makecell{Execution\\time} &
    \makecell{Total\\time$^\perp$} &
    \makecell{\#Expanded\\nodes} &
    \makecell{\#Sub\\plans} \\ \hline\hline
    
    \multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{Sorting Objects}}} &
    \multirow{3}{*}{1} &
    \multirow{3}{*}{20} &
    \multirow{3}{*}{2} &
    \multirow{3}{*}{High} &
    \textbf{Lazy-SIIW}$_{\boldsymbol{R}}$ &
    100\% &
    3.16~\si{\minute} &
    3.67~\si{\minute} &
    6.83~\si{\minute} &
    60 &
    14 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    SIW$_R$ &
    100\% &
    13.05~\si{\minute} &
    3.73~\si{\minute} &
    16.78~\si{\minute} &
    54 &
    14 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    BFWS &
    100\% &
    5.25~\si{\minute}$^*$ &
    5.91~\si{\minute} &
    11.16~\si{\minute}&
    63.3k &
    1 \\ \cline{2-12}

    &
    \multirow{3}{*}{3} &
    \multirow{3}{*}{25} &
    \multirow{3}{*}{5} &
    \multirow{3}{*}{Medium} &
    \textbf{Lazy-SIIW}$_{\boldsymbol{R}}$ &
    100\% &
    3.36~\si{\minute} &
    3.95~\si{\minute} &
    7.31~\si{\minute} &
    235 &
    10 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    SIW$_R$ &
    100\% &
    21.60~\si{\minute} &
    4.02~\si{\minute} &
    25.62~\si{\minute} &
    198 &
    10 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    BFWS &
    100\% &
    13.47~\si{\minute}$^*$ &
    7.61~\si{\minute} &
    21.08~\si{\minute} &
    3.5k &
    1 \\ \cline{2-12}

    &
    \multirow{3}{*}{4} &
    \multirow{3}{*}{28} &
    \multirow{3}{*}{14} &
    \multirow{3}{*}{Medium} &
    \textbf{Lazy-SIIW}$_{\boldsymbol{R}}$ &
    100\% &
    6.52~\si{\minute} &
    9.24~\si{\minute} &
    15.76~\si{\minute} &
    630 &
    34 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    SIW$_R$ &
    100\% &
    47.38~\si{\minute} &
    9.17~\si{\minute} &
    56.55~\si{\minute} &
    587 &
    34 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    Planet &
    N/A &
    $>$1~\si{h} &
    $\approx$10~\si{\minute} &
    $>$1~\si{h} &
    N/A &
    1 \\ \hline\hline

    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\makecell{Non-\\Mono.}}}} &
    \multirow{2}{*}{2} &
    \multirow{2}{*}{10} &
    \multirow{2}{*}{10} &
    \multirow{2}{*}{Low} &
    \textbf{Lazy-SIIW}$_{\boldsymbol{R}}$ &
    100\% &
    3.53~\si{\minute} &
    8.10~\si{\minute} &
    11.63~\si{\minute} &
    565 &
    30 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    SIW$_R$ &
    100\% &
    17.69~\si{\minute} &
    7.96~\si{\minute} &
    25.65~\si{\minute} &
    534 &
    30 \\ \hline\hline

    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\makecell{Blocks\\World}}}} &
    \multirow{2}{*}{1} &
    \multirow{2}{*}{11} &
    \multirow{2}{*}{4-5} &
    \multirow{2}{*}{Low} &
    \textbf{Lazy-SIIW}$_{\boldsymbol{R}}$ &
    100\% &
    2.26~\si{\minute} &
    3.49~\si{\minute} &
    5.75~\si{\minute} &
    243 &
    13 \\ \cdashline{6-12}

    &
    &
    &
    &
    &
    SIW$_R$ &
    100\% &
    8.07~\si{\minute} &
    3.58~\si{\minute} &
    11.65~\si{\minute} &
    216 &
    13 \\ \hline
    \end{tabular}
    {\footnotesize    
    \begin{itemize}
      \item[$^\perp$]Considering that the path execution does not start until the path has been completely planned.
      \item[$^*$]Including also the pre-processing time, for a fair comparison.
    \end{itemize}
    }
\end{table*}

\section{Results and Discussion}\label{sec:results}

\nestor{highlight proposed approach is probabilistically complete, unlike other approaches such as BFWS} 

\magi{In Table 1, we compare our approach Lazy-SIIW$_R$ (i.e. Lazy Serialized Incremental Iterated Width with Sketches) with the original SIW$_R$}

The proposed framework has been evaluated in different instances of the selected benchmarking families\footnote{Videos of the obtained plans can be found in  \url{https://drive.google.com/drive/folders/110VtyoSNrw0hjR7Wma7fumqJIB9wxr3L}}, to analyze its performance in various environments but also to allow direct comparison with other approaches in the same scenario.
The framework has been run in an Intel{\small{\textregistered}}~Core\texttrademark~\mbox{i7-10610U CPU} at 1.80~GHz, with 8~processors and 16~Gb of RAM, on Ubuntu 20.04.4 and ROS Noetic, and validated with a TIAGo robot from PAL Robotics (see Figure~\ref{fig:problems}).
The results obtained by the proposed approach, together with the ones of some relevant algorithms, can be found in Table~\ref{tab:solution}.
In addition, to show the improvements introduced by the developed optimizations, it also reports the results obtained by the plain \siwR { }(i.e. with complete action validations in each search step, hence, non-lazy, and without the incremental version of \iw{k}).
% {\color{red} Non-Lazy and non-goal-serialized versions of the approach have also been tested in these same scenarios as a baseline of the performance improvement provided by each of the proposed strategies.
% However, the results obtained without using goal-serialization are not included since these planners cannot solve any problem in the allocated time.}

All the considered problems have been successfully solved within $1~\si{\hour}$.
Note that this budget time, which would not be admissible on a real application, has set intentionally generous to show the soundness and completeness of the algorithm.
During the experimentation, the effectiveness of the planner has been demonstrated by not requiring planning times longer than the execution time of the produced plans. 
Indeed, the proposed approach requires less time to find a solution compared with the results obtained by \emph{BFWS}~\cite{FerrerMestres2017CombinedTA}, which also use a width-based algorithm, and \emph{Planet}~\cite{Thomason}, which performs normal motion planning in a space including both geometric and symbolic states.
Notice that, in order to make a fair comparison, any pre-computation or other planning effort conducted offline are also considered as planning time in Table~\ref{tab:solution}.
Note that the proposed approach specifically avoids this sort of offline work since, in a real application, there is no guarantee that the objects will be in the positions foreseen in the pre-processing, or that objects of different geometry will not be used.
Indeed, even without the proposed optimizations (lazy validation and incremental \iw{k}), introducing the sketch-based serialization has allowed to obtain similar performance with respect to the other authors but avoiding any of the mentioned rigid assumptions. 
% \magi{proposed approach outperformes competitors. indeed, just using sketches outperforms Planet and obtains planning times similar to BFWS (but precomputes, not flexible)}

The planning time depends on both the number of expanded nodes and the required time for expanding each node.
Regarding the first factor, even though the problem search-space is huge, the planner manages to find a solution expanding only a minimal fraction for all the problems.
Consistently with the theoretical explanation given in X, during the experimentation, a novelty of 1 has been enough to solve all the problems.
% Thanks to the used {\color{red} atom features} and sketch rules, {\color{red} a novelty of 1 has been enough to solve all the problems}.
Thus, the underlying IW$(1)$ algorithm applies the maximum level of node-pruning (hence, minimizing the number of expanded nodes).
In addition, the generated decomposition in subproblems has efficiently guided the search by obtaining a sequence of subgoals very close to each other (i.e.~they require limited exploration to reach them consecutively).

\magi{Highlight it more? }
Furthermore, the followed strategy of adaptive sampling allows to use a reduced but useful selection of placements in each subproblem.
With fewer placements, the search-space is reduced but, in addition, as the sampled placements are automatically adapted to the specific situation of the subproblem, the subgoals are reached quickly.

The node-expansion time in the proposed approach mostly depends on the geometric validation of each of the actions.
This includes three steps (i.e.~\mbox{\emph{InArmWorkspace}}, \mbox{\emph{InverseKinematics}} and \mbox{\emph{MotionPlan}}) that act as sequential filters (i.e.~if a step fails, the next ones are not computed and the action is set as unfeasible).
Note that they act in increasing order of computational load and decreasing order of relative discriminative power (i.e.~rejection ratio over the non-filtered actions in the previous step). 
This permits discarding quickly the majority of unfeasible actions with a very small computational cost (see some illustrative values in Table~\ref{tab:profiling}). 
In addition, decomposing the action-validation enables delaying the computation of the most expensive step (i.e.~\emph{MotionPlan}). 
Thus, the complete validation is only computed on those actions that are part of a potential plan {\color{red}(i.e.~\emph{lazy approach})}.
Note that satisfying the \emph{InverseKinematics} step almost ensures that the action is valid.
This is essential to make using the {\color{red}lazy approach} advantageous.
Indeed, as it can be seen on Table~\ref{tab:solution}, following the {\color{red}lazy approach} reduces drastically the planning time. 

Implementing the {\color{red}lazy-approach}, however, implies some challenges.
Since the actions are all provisional (until a plan is validated), all the found parents in each node must be kept to prevent discarding connections that are part of the solution.
Besides, the planner keeps record on node chains that are connected to a goal but got sometime disconnected from the root node within a plan validation. 
These two mechanisms are relevant when many nodes need to be expanded in a subsearch.
Another important challenge is the adaptation of the IW$(k)$ to keep track of the novelty. 
Thus, when a provisional action turns to be unfeasible, if the node becomes orphan (i.e.~disconnected from the root node), the novelty introduced by this node has to be revised. 
Solving the different problems has implied the activation of this mechanism in multiple occasions. 
This has prevented to wrongly prune graph branches that are part of the solution. 

Another important metric is the quality of the produced plans.
Although optimality can not be formally ensured, the proposed algorithm performs notably on avoiding unhelpful actions (i.e.~near-optimal solutions). 
This is facilitated by the proposed sketch since its rules discourages moving non-misplaced objects that do not block any goal object or goal placement but promotes moving the easier goal-objects first.
Hence, after moving these objects, often other goal objects became accessible without needing to move non-goal objects. 
Indeed, when comparing the results with the other approaches, plans containing fewer actions are obtained for the same problems with the proposed approach. 

The proposed algorithm performs well even with a high number of objects and goals.
However, high-cluttered problems are challenging.
On these problems, the goal objects can be obstructed by many objects, which must be moved away. 
Nevertheless, there is a limited space where the obstructing objects could be set aside (without blocking other necessary areas).
In this scenario, most of the inverse-kinematic computations fail, reaching the timeout. 
This implies a slower node expansion and a higher difficulty to find valid actions. 
In addition, as there are so few gaps, the proposed approach samples the placements more densely to ensure that there exists an accessible placement.
On the contrary, Planet does not scale well with the number of objects.
BFWS scales well, though, but at the cost of rigidity as it pre-compiles and forces the objects to be in a fixed grid distribution during the search process.
With this inflexible approach, the planner manages to reuse many inverse-kinematic and motion-planning computation.

\begin{table}[!t]
    \centering
    \caption{Profiling of the action-validation pipeline.}\label{tab:profiling}
    \def\arraystretch{1.4}
    \setlength\tabcolsep{0.8mm}
    \begin{tabular}{|l||c|c|c|c|}
    \hline
    \multicolumn{1}{|c||}{Step / Function} & \makecell{Success\\time} & \makecell{Time-\\out} & \makecell{Rel.\\success} & \makecell{Cumul.\\success} \\ \hline\hline
    1. \emph{InArmWorkspace} & 35~\si{\micro \second} & N/A & 5-30\% & 5-30\% \\ \hline
    2. \emph{InverseKinematics} & 9~\si{\milli \second} & 0.15~\si{\second} & 20-40\% & 1-10\% \\ \hline
    3. \emph{MotionPlan} & 0.38~\si{\second} & 5~\si{\second} & 80-100\% & 0.5-10\% \\ \hline
    \end{tabular}
\end{table}
}

==> sections/sketch_discussion.tex <==

The following features have been implemented:
\begin{itemize}
    \item $H$: a Boolean that equals $\mathrm{true}$ if the robot is holding an object, and $\mathrm{false}$ otherwise.
    
    \item $F$: a Boolean that equals $\mathrm{true}$ if there exists a goal pose of the grasped object that do not blocks the pick/place of any other misplaced object, and $\mathrm{false}$ otherwise.
    
    \item $m$:
    the number of \emph{misplaced} objects, defined as the objects that are standing (and, hence, not held) outside their associated goal position/region (if the object has no associated goal position, it is never misplaced) or are held and their goal position/region is blocked.
    
    \item $n$ and $s$: respectively $\min b_i + c_i$ and $\sum b_i$, with $b_i$ being the minimum number of objects blocking the $i$-th misplaced object (i.e.~preventing it from being picked up from its current position and put down in its goal position/region) and $c_i$ the minimum number of misplaced object blocked by the goal position(s) of the $i$-th misplaced object.\magi{Note that $c_i$ has been added to $n$ computation. As $n$ wants to capture how far to be freely picked and placed is the best(s) (i.e. less blocked) misplaced object(s) it is necessary not only know how many objects are blocking directly the pick or the place but also how many other misplaced are blocked by this misplaced object goal. Thus $n_i$ capture how many other misplaced objects should be moved before the misplaced object can be placed in its goal }
    Note that approximations are used and no inverse kinematics is solved within this computation, to speed up the process.
    During the search for such a minimum value, it is considered the best robot location and grasp for the \emph{pick} action and the best robot location, object placement and SOP for the \emph{place} action in the goal zone, while maintaining consistency (i.e.~using the same grasp for the considered \emph{pick} and \emph{place} pair).
\end{itemize}

Using these features, the goal in both family problems is expressed as~$\neg H \wedge m=0$ (i.e.~the robot is not holding any object and all the objects are at their goal positions). 
In adition, the following mutually-exclusive sketch rules have been established for both benchmarking problem families:
\begin{itemize}
    \item $\{\neg H,\, m>0,\, n=0 \} \mapsto \{H,\, F,\, m\!\downarrow,\, n?,\, s?\}$:
    active if there is at least one misplaced object ($m>0$) that can be picked up and placed down directly ($\neg H$ and $n=0$), enforcing to pick it up (i.e.~lower~$m$ and make~$H$ \textrm{true}). \magi{F has been included in the rhs of the rule to ensure that the object picked can be placed in its goal without blocking any other misplaced}
    
    \item $\{ \neg H,\, m>0,\, n>0 \} \mapsto \{ H,\, F?,\, m?,\, n?,\, s\!\downarrow \}$:
    active if there are still misplaced objects ($m>0$) but they cannot be picked up directly ($\neg H$ but $n>0$), enforcing to pick any obstructing object (i.e.~decrement~$s$).
    However, $n$ may be accurately estimated, picking an unexpectedly-accessible misplaced object would also satisfy this rule (which is not an inconvenience at all).
    
    \item $\{ H,\, F \} \mapsto \{ \neg H,\, F? \}$:
    active whenever the robot is holding an object, which would not block other misplaced object once placed if it had a goal associated with it, enforcing to place it but not in a wrong position (i.e.~do not change~$m$) and without disturbing the access to the pending misplaced objects (do not change $n$ or $s$).

    \item $\{ H,\, \neg F \} \mapsto \{ \neg H,\, F?,\, m?\}$:
    active whenever the robot is holding an object that cannot be placed on their goal without blocking any misplaced object, enforcing to place it somewhere else without disturbing the access to the pending misplaced objects (do not change $n$ or $s$).
\end{itemize}

